Welfare Distribution in Two-sided Random Matching Markets

We study the welfare structure in two-sided large random matching markets. In the model, each agent has a latent personal score for every agent on the other side of the market and her preferences follow a logit model based on these scores. Under a contiguity condition, we provide a tight description of stable outcomes. First, we identify an intrinsic fitness for each agent that represents her relative competitiveness in the market, independent of the realized stable outcome. The intrinsic fitness values correspond to scaling coefficients needed to make a latent mutual matrix bi-stochastic, where the latent scores can be interpreted as a-priori probabilities of a pair being matched. Second, in every stable (or even approximately stable) matching, the welfare or the ranks of the agents on each side of the market, when scaled by their intrinsic fitness, have an approximately exponential empirical distribution. Moreover, the average welfare of agents on one side of the market is sufficient to determine the average on the other side. Overall, each agent's welfare is determined by a global parameter, her intrinsic fitness, and an extrinsic factor with exponential distribution across the population.

==> approx_stable.tex <==

\section{Generalization to approximately stable matchings}\label{Sec_approx_stable}

Exact stability is an arguably overly stringent requirement. 
analysis can be further extended to understand behaviors of matchings that are approximately stable in the following perspective.

\begin{definition}
We say a matching $\mu$ between $\cM$ and $\cW$ is $\alpha$-stable for some $0 < \alpha < 1$ if there exists a sub-market of size at least $(1-\alpha) n$ on which $\mu$ is stable; that is, there exist subsets $\cM'\subseteq \cM$ and $\cW' \subseteq \cW$ both with cardinality $|\cM'|=|\cW'| \ge (1-\alpha) n$ such that $\mu(\cM') = \mu(\cW')$ and the partial matching induced by $\mu$ between $\cM'$ and $\cW'$ is stable (within this sub-market). We refer to the stable sub-matching between $\cM'$ and $\cW'$ as the \emph{stable part} of $\mu$.
Denote the set of $\alpha$-stable matchings by $\mathcal{S}_\alpha$.
\end{definition}

A simple adaptation of our previous results and proofs for fully stable matchings gives the following Theorem, analogous to Theorem~\ref{Thm_main_happiness_dist_body} and \ref{Thm_main_rank_dist_body}.



\begin{theorem}\label{Thm_dist_body_approx_stable}
    Assume $\alpha = \alpha(n)$ is such that $h(\alpha) > n^{-\eta}$ for some constant $\eta > 0$. Then, for any fixed $\eps > 0$,
    \begin{equation}\label{Eqn_happiness_dist_approx_stable}
        \Pp\bigg(\max_{\mu\in\mathcal{S}_\alpha} \inf_{\lambda\in\R_+} \|\Femp(\vX(\mu))-F_\lambda\|_\infty \le \eps\bigg) \to 1 \text{ as } n\to\infty,
    \end{equation}
    and
    \begin{equation}\label{Eqn_rank_dist_approx_stable}
        \Pp\bigg(\max_{\mu\in\mathcal{S}_\alpha} \inf_{\lambda\in\R_+} \|\Femp(\bm{\phi}^{-1}\circ\mathbf{R}(\mu))-F_\lambda\|_\infty \le \eps\bigg) \to 1 \text{ as } n\to\infty,
    \end{equation}
    where $\phi_i = \sumjton a_{ij}$.
\end{theorem}

The proof is straightforward and is deferred to Appendix~\ref{appendix_extra_proofs}. The key observation is that, if the entire market satisfies the cohesion assumption, then each sub-market of it is also cohesive, and we can apply union bound over all sub-markets of size $(1-\alpha)n$. This argument goes through even when the market is imbalanced.

As an immediate corollary, we have the following result for slightly imbalanced markets.

\begin{corollary}\label{Cor_body_imbalance}
    Consider a market consisting of $n-k$ men and $n$ women, where $h_b(k/n) > n^{-\eta}$ for some constant $\eta > 0$. Assume that the cohesion condition holds as in Assumption~\ref{Assumption_C_bounded}, i.e., the pairwise scores are bounded on $[1/C, C]$. Then, for any fixed $\eps > 0$,
    \begin{equation}\label{Eqn_happiness_dist_imbalance}
        \Pp\bigg(\max_{\mu\in\mathcal{S}} \inf_{\lambda\in\R_+} \|\Femp(\vX(\mu))-F_\lambda\|_\infty \le \eps\bigg) \to 1 \text{ as } n\to\infty,
    \end{equation}
    and
    \begin{equation}\label{Eqn_rank_dist_imbalance}
        \Pp\bigg(\max_{\mu\in\mathcal{S}} \inf_{\lambda\in\R_+} \|\Femp(\bm{\phi}^{-1}\circ\mathbf{R}(\mu))-F_\lambda\|_\infty \le \eps\bigg) \to 1 \text{ as } n\to\infty,
    \end{equation}
    where $\phi_i = \sumjton a_{ij}$.
\end{corollary}
This follows directly from Theorem~\ref{Thm_dist_body_approx_stable} as we can backfill the market with $k$ men with unit scores with all women, so that any stable matching in the original imbalanced market can be extended to an $\frac{k}{n}$-stable matching in the extended market.

\begin{remark}
    The results will not hold if there is a linear imbalance in the market, i.e., $k \propto n$. This is because in such markets the men achieve a constant average rank \cite{ashlagi2017unbalanced}, and therefore the convergence to the exponential distribution is impossible.  
\end{remark}

One should be able to further strengthen the results through a more careful analysis. However, we choose to leave these potentials for future studies. %





    
























